TMIQ: Quantifying Test and Measurement Domain Intelligence in Large Language Models

The Test and Measurement domain, known for its strict requirements for accuracy and efficiency, is increasingly adopting Generative AI technologies to enhance the performance of data analysis, automation, and decision-making processes. Among these, Large Language Models (LLMs) show significant promise for advancing automation and precision in testing. However, the evaluation of LLMs in this specialized area remains insufficiently explored. To address this gap, we introduce the Test and Measurement Intelligence Quotient (TMIQ), a benchmark designed to quantitatively assess LLMs across a wide range of electronic engineering tasks. TMIQ offers a comprehensive set of scenarios and metrics for detailed evaluation, including SCPI command matching accuracy, ranked response evaluation, Chain-of-Thought Reasoning (CoT), and the impact of output formatting variations required by LLMs on performance. In testing various LLMs, our findings indicate varying levels of proficiency, with exact SCPI command match accuracy ranging from around 56% to 73%, and ranked matching first-position scores achieving around 33% for the best-performing model. We also assess token usage, cost-efficiency, and response times, identifying trade-offs between accuracy and operational efficiency. Additionally, we present a command-line interface (CLI) tool that enables users to generate datasets using the same methodology, allowing for tailored assessments of LLMs. TMIQ and the CLI tool provide a rigorous, reproducible means of evaluating LLMs for production environments, facilitating continuous monitoring and identifying strengths and areas for improvement, and driving innovation in their selections for applications within the Test and Measurement industry.

==> latex_bibliography.tex <==
\begin{thebibliography}{99}
\bibitem[1]{} H. L. Fernandez-Canque, Analog Electronics Applications: Fundamentals of Design and Analysis. Boca Raton, FL: CRC Press, 2017.
\bibitem[2]{}  S. W. Smith, The Scientist and Engineer's Guide to Digital Signal Processing, 2nd ed. San Diego, CA: California Technical Publishing, 1999.
\bibitem[3]{} E. A. Lee and S. A. Seshia, Introduction to Embedded Systems - A Cyber-Physical Systems Approach, Second Edition, MIT Press, 2017.
\bibitem[4]{} B. A. Gregory, An Introduction to Electrical Instrumentation and Measurement Systems, 2nd ed. New York, NY, USA: Halsted Press, a Division of John Wiley \& Sons, Inc., 1981.
\bibitem[5]{} D. Placko, Fundamentals of Instrumentation and Measurement. London, UK: ISTE Ltd, 2007.
\bibitem[6]{} R. B. Northrop, Introduction to Instrumentation and Measurements, 2nd ed. Boca Raton, FL, USA: CRC Press, Taylor \& Francis Group, 2005.
\bibitem[7]{} A. S. Morris, Measurement and Instrumentation Principles. Oxford, U.K.: Butterworth-Heinemann, 2001.
\bibitem[8]{} D. Hanes, G. Salgueiro, P. Grossetete, R. Barton, and J. Henry, *IoT Fundamentals: Networking Technologies, Protocols, and Use Cases for the Internet of Things*. Indianapolis, IN, USA: Cisco Press, 2017.
\bibitem[9]{}  R. F. Coughlin and F. F. Driscoll, Operational Amplifiers and Linear Integrated Circuits, 6th ed. Upper Saddle River, NJ: Prentice Hall, 2001.
\bibitem[10]{} Keysight Technologies, The Parametric Measurement Handbook, 4th ed. Santa Rosa, CA: Keysight Technologies, 2020
\bibitem[11]{} B. Razavi, RF Microelectronics. Upper Saddle River, NJ: Prentice Hall, 1998.
\bibitem[12]{} W. A. Davis and K. Agarwal, Radio Frequency Circuit Design. New York, NY, USA: Wiley-Interscience, 2001.
\bibitem[13]{} C. Bowick, RF Circuit Design, 2nd ed. Burlington, MA, USA: Newnes, 2008.
\bibitem[14]{} J. J. Carr, RF Components and Circuits. Oxford, U.K.: Newnes, 2002.
\bibitem[15]{} J. M. Fiore, Semiconductor Devices: Theory and Application, version 1.1.12. Utica, NY, USA: self-published, 2021.
\bibitem[16]{} M. Resso and E. Bogatin, Signal Integrity Characterization Techniques. Chicago, IL, USA: International Engineering Consortium, 2009.
\bibitem[17]{} Sung-Mo Kang and Yusuf Leblebici, *CMOS Digital Integrated Circuits: Analysis and Design*, 2nd ed. Boston, MA, USA: McGraw-Hill, 2003.
\bibitem[18]{} O. Simeone, 'A brief introduction to machine learning for engineers' *arXiv preprint* arXiv:1709.02840, 2018. [Online]. Available: https://arxiv.org/abs/1709.02840.
\bibitem[19]{} V. Quaschning, *Understanding Renewable Energy Systems*. London, U.K. and Sterling, VA, USA: Earthscan, 2005.
\end{thebibliography}
